Analysis and Validation of Image Search Engines in Histopathology

Searching for similar images in archives of histology and histopathology images is a crucial task that may aid in patient matching for various purposes, ranging from triaging and diagnosis to prognosis and prediction. Whole slide images (WSIs) are highly detailed digital representations of tissue specimens mounted on glass slides. Matching WSI to WSI can serve as the critical method for patient matching. In this paper, we report extensive analysis and validation of four search methods bag of visual words (BoVW), Yottixel, SISH, RetCCL, and some of their potential variants. We analyze their algorithms and structures and assess their performance. For this evaluation, we utilized four internal datasets ($1269$ patients) and three public datasets ($1207$ patients), totaling more than $200,000$ patches from $38$ different classes/subtypes across five primary sites. Certain search engines, for example, BoVW, exhibit notable efficiency and speed but suffer from low accuracy. Conversely, search engines like Yottixel demonstrate efficiency and speed, providing moderately accurate results. Recent proposals, including SISH, display inefficiency and yield inconsistent outcomes, while alternatives like RetCCL prove inadequate in both accuracy and efficiency. Further research is imperative to address the dual aspects of accuracy and minimal storage requirements in histopathological image search.

==> conflicts.tex <==
The authors do not have any conflict of interest to declare.

==> contributions.tex <==
IL implemented and validated the SISH and RetCCL search engines and wrote the first draft of the paper. SA designed experiments, analyzed results,  wrote parts of the paper, re-run many experiments and double-checked the results. LK and VK contributed to the experiments by implementing the BoVW approach and verifying results. PN, SA, AA, AS, GA, JK, and SH contributed to the experiments and analysis by testing Yottixel. IL, SA, and PN also contributed to writing the manuscript. NC, DM, AA, SA, CM, LB, VHS, and JJG guided data collection and curation, provided advice for validation. HRT designed the experiments, provided algorithmic guidance, analyzed results, and contributed to writing the manuscript.
